Narwhal and Tusk: A DAG-based Mempool and Efficient BFT Consensus

We propose separating the task of reliable transaction dissemination from transaction ordering, to enable high-performance Byzantine fault-tolerant quorum-based consensus. We design and evaluate a mempool protocol, Narwhal, specializing in high-throughput reliable dissemination and storage of causal histories of transactions. Narwhal tolerates an asynchronous network and maintains high performance despite failures. Narwhal is designed to easily scale-out using multiple workers at each validator, and we demonstrate that there is no foreseeable limit to the throughput we can achieve. Composing Narwhal with a partially synchronous consensus protocol (Narwhal-HotStuff) yields significantly better throughput even in the presence of faults or intermittent loss of liveness due to asynchrony. However, loss of liveness can result in higher latency. To achieve overall good performance when faults occur we design Tusk, a zero-message overhead asynchronous consensus protocol, to work with Narwhal. We demonstrate its high performance under a variety of configurations and faults. As a summary of results, on a WAN, Narwhal-Hotstuff achieves over 130,000 tx/sec at less than 2-sec latency compared with 1,800 tx/sec at 1-sec latency for Hotstuff. Additional workers increase throughput linearly to 600,000 tx/sec without any latency increase. Tusk achieves 160,000 tx/sec with about 3 seconds latency. Under faults, both protocols maintain high throughput, but Narwhal-HotStuff suffers from increased latency.

==> Makefile <==
.PHONY: FORCE lenny all clean distclean

FILE=main

all: $(FILE).pdf

%.pdf: %.tex FORCE
	latexmk -pdf -f -e '$$pdflatex=q/pdflatex %O %S/' $<

fast:
	pdflatex $(FILE)


clean:
	for ext in aux log toc lof lot lol dlog bbl \
		nav snm fls vrb blg out tpt fdb_latexmk; \
	do \
		$(RM) $(FILE).$$ext ; \
	done
	$(RM) *.aux *.bak *~

distclean: clean
	$(RM) $(FILE).pdf
	$(RM) $(FILE).ps
	$(RM) $(FILE).dvi
	$(RM) *.d

read: all
	open $(FILE).pdf


==> sections/A2-hs.tex <==
\section{Comparison with \hotstuff}
\label{sec:hs}

We implement and evaluate two version of \hotstuff, \vanillahs and \batchedhs. \vanillahs implements the classic 3-chain \hotstuff protocol~\cite{DBLP:conf/podc/YinMRGA19}. Instead of using the implementation provided by the authors, we re-implemented it to allow a fairer comparison with our systems (same network, crypto, and storage). We then modify \vanillahs to decouple the mempool from consensus to improve performance. We call this modified system \batchedhs. Both \vanillahs and \batchedhs use a simple round-robin as leader-election mechanism.
We are open sourcing the both our implementations, Amazon web services orchestration scripts, benchmarking scripts, and measurements data to enable reproducible results\footnote{
\ifdefined\cameraReady
\url{https://github.com/asonnino/hotstuff}
\else
Link omitted for blind review.
\fi
}.

\subsection{Experimental setup}
Similarly to \Cref{sec:evaluation}, we evaluate the throughput and latency of our implementations through experiments on AWS. We  particularly aim to highlight the tradeoffs with \sysname.
%
For each implementation, we deploy a testbed on Amazon Web Services, using \texttt{m5.8xlarge} instances scattered across 4 different AWS regions: N. Virginia (us-east-1), N. California (us-west-1), Sydney (ap-southeast-2), and Stockholm (eu-north-1). This class of instance provides 10 Gbps of bandwidth, 32 virtual CPUs (16 physical core) on a 2.5 GHz, Intel Xeon Platinum 8175, and 128 GB memory. The operating system is Linux Ubuntu server 20.04.

In the following sections, each measurement in the graphs is the average of 2 runs, and the error bars represent one standard deviation. Our baseline experiment parameters are: a transaction size of 512B, and one benchmark client per node submitting transactions at a fixed rate for a duration of 5 minutes. We vary the batch size from 200 transactions (when the system is under low load) to 1,000 transactions (when the system is under high load) to optimize performance.

\subsection{Comparison with \vanillahs}
\alberto{TODO}

\subsection{Comparison with \batchedhs}
\batchedhs separates the mempool from consensus. The mempool receives clients’ transactions, batches them into payloads (of configurable size) and broadcasts them to other nodes; we may call these messages 'mempool batches'. Their purpose is to disseminate client's transactions to the other nodes before consensus attempts to sequence them (thus allowing a more egalitarian bandwidth utilization among nodes). They also reduce client-perceived latency as a node does not necessarily need to wait to become leader to propose the transactions of their clients: other nodes may include their transactions after receiving them as part of mempool batches.

Consensus is then reached on the hashes of these mempool batches. Whenever consensus needs to create a block proposal, it queries its local mempool for the hashes of one or many payloads to include in its block. Its query specifies a maximum number of bytes it wishes to receive so to ensure an upper bound on the size of its proposals. We experimentally found that setting this maximum to 1KB gives the best performance. The mempool replies to consensus with as many hashes of payloads as possible (while respecting the size constraint in the query), but may also reply with an empty vector in case there are no payloads available. 


\para{Evaluation in the happy-path}
\Cref{fig:hs-latency} illustrates the latency-throughput graph of \sysname for various committee sizes. Figures~\ref{fig:hs-tps} and~\ref{fig:hs-robustness} illustrate the throughput for various committee sizes. These graphs show that both the throughput and latency of \batchedhs are about half of \sysname.
\alberto{Should we describe the graphs more?}

Under high load, there is a probability that one node (usually the one in Australia, that is the most isolated from the rest of the network) falls behind and never manages to sync up with the others. When this happens, latency greatly increases and throughput decreases since the slow node keeps being elected as leader and is slow to propose. The higher the input rate, the greater the probability that one node falls behind. This is why we see sometimes huge error bars in the graphs: performance is good during ``lucky runs'' when all nodes stay synchronized, but tumble when they don't. We also observe that there is a fairly neat threshold of input rate over which the probability that one node falls behind increases (e.g., the threshold is around 65,000 tx/s for 20 nodes). %The sensitivity to that threshold is also why performance with 4 nodes is much lower than with 20 nodes: the threshold is pushed back with larger networks because more nodes share the total load.
Figures~\ref{fig:consensus-latency-committee} and~\ref{fig:consensus-robustness-committee} show that \sysname does not suffer from this drawback.


Manually analyzing the logs, we found that catching up on missed consensus blocks is very fast and rarely needed; a lot of time (sometimes over 20 sec) is however spent by the mempool to catch up on missing payloads. What desynchronizes the node in Australia is missing past payloads. These observations outline the importance of building a performant mempool.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.47\textwidth]{figures/vanilla-hs-latency}
    \caption{Latency-throughput graph of \vanillahs for various committee sized. The transaction size is set to 512 B, and the batch size varies from 200 to 1,000 transactions.}
    \label{fig:vanilla-hs-latency}
\end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.47\textwidth]{figures/vanilla-hs-tps}
    \caption{Throughput of \vanillahs for various committee sizes. The transaction size is set to 512 B, and the batch size varies from 200 to 1,000 transactions.}
    \label{fig:vanilla-hs-tps}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.47\textwidth]{figures/batched-hs-latency}
    \caption{Latency-throughput graph of \batchedhs for various committee sized. The transaction size is set to 512 B, and the batch size varies from 200 to 1,000 transactions.}
    \label{fig:batched-hs-latency}
\end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.47\textwidth]{figures/batched-hs-tps}
    \caption{Throughput of \batchedhs for various committee sizes. The transaction size is set to 512 B, and the batch size varies from 200 to 1,000 transactions.}
    \label{fig:batched-hs-tps}
\end{figure}


%\begin{figure}[t]
%    \centering
%    \includegraphics[width=0.47\textwidth]{figures/hs-robustness}
%    \caption{Best achievable throughput of \batchedhs while keeping the latency below 4 and 1.2 seconds. The transaction size is set to 512 B, and the batch size varies from 200 to 1,000 transactions.}
%    \label{fig:hs-robustness}
%\end{figure}

\com {
\para{Evaluation under faults}

\lefteris{TODO: Make throughput log-scale }
Figures~\ref{fig:hs-latency-faults} and~\ref{fig:hs-robustness-faults} show the performance of a deployment of \batchedhs with 10 nodes out of which some are crashed. The graphs show that \batchedhs performs extremely poorly under faults; even with a single dead node, \batchedhs's latency grows by a factor of 15 and its throughput decreases by a factor of 10.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.47\textwidth]{figures/hs-latency-faults}
    \caption{Throughput of \batchedhs with 10 nodes out of which some are crashed. The transaction and batch size are respectively set to 512 B and 1,000 transactions.}
    \label{fig:hs-latency-faults}
\end{figure}
%\begin{figure}[t]
%    \centering
%    \includegraphics[width=0.47\textwidth]{figures/hs-robustness-faults}
%    \caption{Throughput of \batchedhs with 10 nodes out of which some are crashed. The transaction and batch size are respectively set to 512 B and 1,000 transactions.}
%    \label{fig:hs-robustness-faults}
%\end{figure}
}

==> sections/A3-sim.tex <==
\section{Discrete event simulator}
\label{sec:sim}

 \begin{figure*}[t!]
     \centering
      \includegraphics[width=0.80\textwidth]{figures/merge.png}
     \caption{ Simulated bandwidth and CPU usage for one node participating in HotStuff (top) or the \sysname mempool protocol (bottom). Observe that in the case of HotStuff a validator saturates their network only when they are leaders, whereas in \sysname network utilization is always high. }
     \label{fig:merge}
\end{figure*}

As part of the \sysname design effort we built a discrete event simulator using 
the Python 3 \texttt{simpy} package to study the bottlenecks in consensus systems. 
Two types of resources were simulated with bounded capacity at each validator: CPU 
and network bandwidth. These resources were designed such that use up to their capacity 
at each validator would only incur a fixed latency, but use exceeding this capacity would 
lead to queuing and increased latency. 

We implemented a model of the HotStuff~\cite{DBLP:conf/podc/YinMRGA19} as implemented 
by the LibraBFT~\cite{baudet2019state} system. The consensus algorithm works in three distinct phases in each round:
\begin{enumerate}
    \item The leader sends proposed blocks to all validators. This phase uses the network at the leader fully, and at other validators only partially. The more validators the lower the network utilization of non-leaders. No CPU is used (except at leader who has proposal first).
    \item Validators pre-execute proposed block to get a state commitment, and vote on it. The network is completely idle in this phase.
    \item Validators send votes and wait for a QC and next vote. Network utilization is minimal, and no CPU is used in this phase, which consists largely of waiting.
\end{enumerate}
Further, the LibraBFT mempool design results in all transactions being send around the network twice. First all validators share individual transactions in the shared mempool protocol, which end up in the future leaders. Subsequently, the leader re-sends all transactions as part of the block proposal.

In summary, despite all theoretical works stressing that bandwidth is the limiting factor for consensus protocols, what we observed through the simulation is that at most validators bandwidth was grossly underutilized most of the time. The exception being the bandwidth at each leader, which was a bottleneck as throughput increased leading to unacceptable latency. Top of \Cref{fig:merge} illustrates this, showing that the bandwidth (blue) is mostly not used, except then the validator becomes leader, which happens in 25\% of slots for 4 validator networks.

Based on these early findings, we simulated a first variant of \sysname and \sysname-HS: we replaced the mempool with a DAG based causal graph of blocks containing transactions and links to past blocks. HotStuff leaders only proposed links to blocks. We observed network utilization close to 100\%, also illustrated in the bottom of \cref{fig:merge}. Thus we extended the design to enable garbage collection, through rounds in \sysname, and sharding through workers, as well as a full evaluation on WAN using Rust, a performant systems language.

==> sections/async.tex <==
\section{Asynchronous SMR}
\label{app:async}


\sasha{TODO: take pseudocode and description from ``all you need is
DAG'' and adjust.}



\paragraph{Liveness proof}
We are going to show that if the leader is unpredictable at round $r+1$ then there are at least $f+2$ candidate leaders that have $f+1$ support in the local DAG of a validator.

The goal of the adversary is to minimize the number of candidate leader with sufficient support. He is tasked to add $2f+1$ unique links of the $2f+1$ blocks of round $r+1$ in at most $3f+1$ candidate blocks of round $r$. His best strategy is to fill all $3f+1$ slots with $f$ links. This is $3f^2+f$ links out of the $4f^2+4f+1$ links hence there are $f^2+3f+1$ more links that by the pidgeonhole principle will force some candidate leaders to gain enough support. 
Once a leader has enough support the adversary's best practice is to maximize the number of links to this leader, hence add all $2f+1$ (there are only $2f+1$ blocks in the DAG of the validator at round $r+1$). As a result, the minimum number of candidate leaders with sufficient support is $\lceil{\frac{f^2+3f+1}{f+1}}\rceil = f+2$.

\lefteris{Safety proofs same as PODC paper}
